Learning the Target Network in Function Space

We focus on the task of learning the value function in the reinforcement learning (RL) setting. This task is often solved by updating a pair of online and target networks while ensuring that the parameters of these two networks are equivalent. We propose Lookahead-Replicate (LR), a new value-function approximation algorithm that is agnostic to this parameter-space equivalence. Instead, the LR algorithm is designed to maintain an equivalence between the two networks in the function space. This value-based equivalence is obtained by employing a new target-network update. We show that LR leads to a convergent behavior in learning the value function. We also present empirical results demonstrating that LR-based target-network updates significantly improve deep RL on the Atari benchmark.

==> sections/old_proof.tex <==
\section{Old result in Appendix A}

We conclude this part with the following result.
\begin{lemma}\label{lem:interm3_strong-temp}
Let $\left\{ (\theta^{t} , w^{t}) \right\}_{t \in \mathbb{N}}$ be a sequence generated by the Lookahead-Replicate algorithm. Choose $\alpha=1/L$. Then, for all $t \in \mathbb{N}$, we have 
\begin{equation*}
\left\|w^{t+1}-w^{\star}\right\|^2 \leq (1-\kappa)^{\KL}\left\|w^{t}-w^{\star}\right\|^2+\eta^{2}\left(1 - \left(1 - \kappa\right)^{\KL}\right)\left\|\theta^t-\theta^{\star}\right\|^2,
\end{equation*}
where $\kappa := L^{-1}F_w$ and $\eta := F_w^{-1} F_\theta$.
\end{lemma}
\begin{proof}
Let $t \in \mathbb{N}$. From Proposition \ref{lem:interm2_strong} (recall that $\alpha = 1/L$) and the fact that $w^{t + 1} = w^{t , \KL}$, we have 
\begin{align*}
 \left\|w^{t+1}-w^{\star}\right\|^2 & =\left\|w^{t, \KL}-w^{\star}\right\|^2 \\
 & \leq(1-\kappa)\left\|w^{t, \KL-1}-w^{\star}\right\|^2+\eta^2 \kappa\left\|\theta^t-\theta^{\star}\right\|^2 \\
& \leq(1-\kappa)\left[(1-\kappa)\left\|w^{t, \KL-2}-w^{\star}\right\|^2+\eta^2 \kappa\left\|\theta^t-\theta^{\star}\right\|^2\right]+\eta^2 \kappa\left\|\theta^t-\theta^{\star}\right\|^2 \\
& =(1-\kappa)^2\left\|w^{t, \KL-2}-w^{\star}\right\|^2+\eta^2 \kappa(1+(1-\kappa))\left\|\theta^t-\theta^{\star}\right\|^2 \\
& \leq \cdots \\
& \leq(1-\kappa)^{\KL}\left\|w^{t, 0}-w^{\star}\right\|^2+\eta^2 \kappa \sum_{k=0}^{\KL-1}(1-\kappa)^k\left\|\theta^t-\theta^{\star}\right\|^2 \\
& =(1-\kappa)^{\KL}\left\|w^{t}-w^{\star}\right\|^2+\eta^2 \kappa \sum_{k=0}^{\KL-1}(1-\kappa)^k\left\|\theta^t-\theta^{\star}\right\|^2,
\end{align*}
where the last inequality follows from the fact that $w^{t,0} = w^{t}$. Because $\kappa\in[0,1]$, the geometric series on the right hand side is convergent, and so we can write:
\begin{equation*}
    \eta^2 \kappa \sum_{k = 0}^{\KL - 1} \left(1 - \kappa\right)^{k} = \eta^2 \kappa \frac{1 - \left(1 - \kappa\right)^{\KL}}{1 - \left(1 - \kappa\right)} = \eta^{2}\left(1 - \left(1 - \kappa\right)^{\KL}\right),
\end{equation*}
which completes the desired result.
\end{proof}


\iffalse
Because $\kappa \in [0,1]$, the geometric series on the right hand side is convergent, and so we can write
\begin{align*}
 \left\|w^{t+1}-w^{\star}\right\|^2 & \leq (1-\kappa)^{\KL}\left\|w^{t}-w^{\star}\right\|^2+\eta^2 \kappa \sum_{k=0}^{\KL-1}(1-\kappa)^k\left\|\theta^t-\theta^{\star}\right\|^2\\
\leq& (1-\eta^2)\norm{\theta^t-\theta^\star}^2 +\eta^2 \kappa \sum_{k=0}^{\KL-1}(1-\kappa)^k\left\|\theta^t-\theta^{\star}\right\|^2\\
=&\left[(1-\eta^2)+\eta^2\left(1-(1-\kappa)^{\KL}\right)\right]\norm{\theta^t-\theta^{\star}}^2
\end{align*}

Note recall the definition in Assumption~\ref{assum1}, it automatically holds $\kappa=F_w/L_w<1$ ($\kappa=1$ is the trivial case), so for any $t\in\NN$, there exists $K_L^t$ such that 
\[
(1-\kappa)^{K^t_L}\norm{w^t - w^\star}^2\leq (1-\eta^2)\norm{\theta^t-\theta^\star}^2.
\] 
To show the above, there are two cases. (i) If $\norm{w^t - w^\star}^2=0$, then any $K_L^t$ satisfies the condition; (ii) if $\norm{w^t - w^\star}^2>0$, since $0\leq \kappa<1$, we can choose any $K_L^t\geq \log(\frac{(1-\eta^2)\norm{\theta^t-\theta^\star}^2}{\norm{w^t-w^\star}^2})/\log(1-\kappa)$
and this implies $(1-\kappa)^{K^t_L}\norm{w^t - w^\star}^2\leq (1-\eta^2)\norm{\theta^t-\theta^\star}^2$.
\begin{align*}
    \lambda_{min}(\Phi^{\top}D\Phi)\norm{w^{t} - w^{\star}}^{2} \leq \norm{v_{w^{t}} - v_{w^{\star}}}_{D}^{2} = \norm{v_{w^{t}} - v_{\theta^{\star}}}_{D}^{2}
\end{align*}
\fi


we will first prove three auxiliary results that are a slight modification of results from the recent paper \cite{asadi2023td}. Since this paper focuses on the analysis of the TD algorithm,
The modification that is needed here motivated by the fact that in this paper we are focusing on RL algorithms that find solutions in the set $\mathcal{F}_{value}$. 







% \begin{theorem}\label{thm:interm3_strong}
% Given Assumption~\ref{assum1}. Let $\left\{\theta^t,w^t\right\}_{t \in \mathbb{N}}$ to a sequence generated by Algorithm~\ref{alg:main} and $(\theta^\star,w^\star)\in\mathcal{F}_{value}$, i.e. $v_{\theta^\star}=v_{w^\star}$ and $v_{w^\star}=\mathcal{T}v_{\theta^\star}$. Suppose $F_w>\max\{F_\theta,2\kappa_1^2\sigma_K\}$, then choose $\beta=\min\{\frac{F_w-2\kappa_1^2\sigma_K}{2(1+\sigma_K)^2\kappa_1^4},\frac{1}{F_w-2\kappa_1^2\sigma_K}\}$, we have
% \[
% \norm{\theta^{t+1}-\theta^\star}^2\leq \bar{\kappa}\norm{\theta^{t}-\theta^\star}^2
% \]
% with $\bar{\kappa}=\max\{\frac{1}{2},1-\frac{\beta(F_w-2\kappa_1^2\sigma_K)}{2}\}<1$ and $\sigma_K$ defined in Lemma~\ref{lem:interm3_strong}.
% \end{theorem}

% \begin{proof}[Proof of Theorem~\ref{thm:interm3_strong}]
% From
% $\theta^{t+1}:=\theta^t - \beta\cdot \EE_\rho[(v_{\theta^t}-v_{w^{t+1}})\nabla v_{\theta^t}]
% $, we have 
% \begin{equation}\label{eqn:strong_main}
% \begin{aligned}
% \norm{\theta^{t+1}-\theta^\star}^2=&\norm{\theta^t-\theta^\star - \beta\cdot \EE_\rho[(v_{\theta^t}-v_{w^{t+1}})\nabla v_{\theta^t}]}^2\\
% =&\norm{\theta^t-\theta^\star}^2-2\beta (\theta^t-\theta^\star)^\top\EE_\rho[(v_{\theta^t}-v_{w^{t+1}})\nabla v_{\theta^t}]+\beta^2\norm{\EE_\rho[(v_{\theta^t}-v_{w^{t+1}})\nabla v_{\theta^t}]}^2\\
% =&\norm{\theta^t-\theta^\star}^2-2\beta (\theta^t-\theta^\star)^\top\EE_\rho[(v_{\theta^t}-v_{\theta^{\star}})\nabla v_{\theta^t}]-2\beta (\theta^t-\theta^\star)^\top\EE_\rho[(v_{w^\star}-v_{w^{t+1}})\nabla v_{\theta^t}]\\
% +&\beta^2\norm{\EE_\rho[(v_{\theta^t}-v_{w^{t+1}})\nabla v_{\theta^t}]}^2,
% \end{aligned}
% \end{equation}
% where the last equal sign uses exactly $v_{\theta^\star}=v_{w^\star}$.
% Then apply the strong convexity condition for $\theta=\theta^\star$, $w_1=\theta^t$ and $w_2=\theta^\star$, we obtain
% \begin{equation}\label{eqn:s_proof1}
% \begin{aligned}
%  F_w\left\|\theta^t-\theta^\star\right\|^2 \leq &\left(\nabla_w H\left(\theta^\star, \theta^t\right)-\nabla_w H\left(\theta^\star, \theta^\star\right)\right)^{\top}\left(\theta^t-\theta^\star\right)\\
%  =&\nabla_w H\left(\theta^\star, \theta^t\right)^{\top}\left(\theta^t-\theta^\star\right)\\
%  =&2(\theta^t-\theta^\star)^\top\EE_\rho[(v_{\theta^t}-v_{\theta^{\star}})\nabla v_{\theta^t}]
% \end{aligned}
% \end{equation}
% where the first equal sign is from $\nabla_w H\left(\theta^\star, \theta^\star\right)=2\EE_\rho[(v_{\theta^\star}-\mathcal{T}v_{\theta^\star})\nabla v_{\theta^\star}]=2\EE_\rho[(v_{w^\star}-\mathcal{T}v_{\theta^\star})\nabla v_{\theta^\star}]=0$.
% Here to obtain $2\EE_\rho[(v_{w^\star}-\mathcal{T}v_{\theta^\star})\nabla v_{\theta^\star}]=0$ we use that $v_{w^\star}=\mathcal{T}v_{\theta^\star}$, which is part of ${\cal F}_{value}$,
% and the second equal sign comes from
% \begin{align*}
% \nabla_w H\left(\theta^\star, \theta^t\right)=2\EE_\rho[(v_{\theta^t}-\mathcal{T}v_{\theta^\star})\nabla v_{\theta^t}]=2\EE_\rho[(v_{\theta^t}-v_{w^\star})\nabla v_{\theta^t}]=2\EE_\rho[(v_{\theta^t}-v_{\theta^\star})\nabla v_{\theta^t}].
% \end{align*}
% Again, to obtain $2\EE_\rho[(v_{\theta^t}-\mathcal{T}v_{\theta^\star})\nabla v_{\theta^t}]=2\EE_\rho[(v_{\theta^t}-v_{w^\star})\nabla v_{\theta^t}]$ we use that $v_{w^\star}=\mathcal{T}v_{\theta^\star}$ which is part of ${\cal R}$. Next,
% \begin{equation}\label{eqn:s_proof2}
% \begin{aligned}
% & (\theta^t-\theta^\star)^\top\EE_\rho[(v_{\theta^\star}-v_{w^{t+1}})\nabla v_{\theta^t}]=(\theta^t-\theta^\star)^\top\EE_\rho[(v_{w^\star}-v_{w^{t+1}})\nabla v_{\theta^t}]\\
%  \leq& \norm{\theta^t-\theta^\star}\cdot \kappa_1^2 \norm{w^\star-w^{t+1}}\leq \kappa_1^2 \sigma_K \norm{\theta^t-\theta^\star}^2,
% \end{aligned}
% \end{equation}
% where the last inequality uses Lemma~\ref{lem:interm3_strong}. Finally, 
% \begin{equation}\label{eqn:s_proof3}
% \begin{aligned}
% &\norm{\EE_\rho[(v_{\theta^t}-v_{w^{t+1}})\nabla v_{\theta^t}]}\leq \norm{\EE_\rho[(v_{\theta^t}-v_{\theta^{\star}})\nabla v_{\theta^t}]}+\norm{\EE_\rho[(v_{w^\star}-v_{w^{t+1}})\nabla v_{\theta^t}]}\\
% \leq&
% \kappa_1^2(\norm{\theta^t-\theta^{\star}}+\norm{w^\star-w^{t+1}})\leq (1+\sigma_K)\kappa_1^2 \norm{\theta^t-\theta^{\star}}
% \end{aligned}
% \end{equation}
% Plug \eqref{eqn:s_proof1}, \eqref{eqn:s_proof2}, \eqref{eqn:s_proof3} back to \eqref{eqn:strong_main} to obtain 
% \begin{align*}
% \norm{\theta^{t+1}-\theta^\star}^2=&\norm{\theta^t-\theta^\star}^2-2\beta (\theta^t-\theta^\star)^\top\EE_\rho[(v_{\theta^t}-v_{\theta^{\star}})\nabla v_{\theta^t}]-2\beta (\theta^t-\theta^\star)^\top\EE_\rho[(v_{w^\star}-v_{w^{t+1}})\nabla v_{\theta^t}]\\
% +&\beta^2\norm{\EE_\rho[(v_{\theta^t}-v_{w^{t+1}})\nabla v_{\theta^t}]}^2\\
% \leq & \norm{\theta^t-\theta^\star}^2-\beta F_w \left\|\theta^t-\theta^\star\right\|^2+2\beta \kappa_1^2 \sigma_K \norm{\theta^t-\theta^\star}^2+\beta^2(1+\sigma_K)^2\kappa_1^4 \norm{\theta^t-\theta^{\star}}^2\\
% =&\norm{\theta^t-\theta^\star}^2-\beta\left(F_w-2\kappa_1^2\sigma_K-\beta(1+\sigma_K)^2\kappa_1^4\right)\norm{\theta^t-\theta^\star}^2\\
% \leq & (1-\frac{\beta(F_w-2\kappa_1^2\sigma_K)}{2})\norm{\theta^t-\theta^\star}^2=\max\{\frac{1}{2},1-\frac{\beta(F_w-2\kappa_1^2\sigma_K)}{2}\}\norm{\theta^t-\theta^\star}^2,
% \end{align*}
% where the last inequality uses $\beta\leq \frac{F_w-2\kappa_1^2\sigma_K}{2(1+\sigma_K)^2\kappa_1^4}$ and the last equality uses $\beta\leq\frac{1}{F_w-2\kappa_1^2\sigma_K}$.

% \end{proof}
We recall that here we analyze the Lookahead-Replicate algorithm for a general value functions $v_{\theta}$ and $v_{w}$ for which the corresponding loss functions
\main*
\begin{proof}
First note that $\nabla_w \norm{v_{w}-\mathcal{T}v_{\theta}}_\rho^2=2\nabla v_w D (v_w-\mathcal{T}v_\theta)$, where $\nabla v_w\in\RR^{d\times S},D=\text{diag}(\rho)\in\RR^{S\times S},v_w-\mathcal{T}v_\theta\in\RR^{S\times 1}$. Similarly, $\nabla_\theta \norm{v_{w}-v_{\theta}}_\rho^2=2\nabla v_\theta D (v_w-v_\theta)$.

From the main step of the Replicate operation (see step 3), we have that  $\theta^{t,k+1} = \theta^{t,k} - 2\beta\cdot \nabla v_{\theta^{t,k}} D (v_{\theta^{t,k}}-v_{w^{t+1}})$. Using this relation yields the following
\begin{align} \label{eqn:strong_main-temp}
\norm{\theta^{t,k+1}-\theta^\star}^2 & = \norm{\theta^{t,k}-\theta^\star - 2\beta\cdot \nabla v_{\theta^{t,k}} D (v_{\theta^{t,k}}-v_{w^{t+1}})}^2 \nonumber\\
& =\norm{\theta^{t,k}-\theta^\star}^2-2\beta (\theta^{t,k}-\theta^\star)^\top \nabla v_{\theta^{t,k}} D (v_{\theta^{t,k}}-v_{w^{t+1}})+\beta^2\norm{\nabla v_{\theta^{t,k}} D (v_{\theta^{t,k}}-v_{w^{t+1}})}^2 \nonumber \\
& =\norm{\theta^{t,k}-\theta^\star}^2-2\beta (\theta^{t,k}-\theta^\star)^\top\nabla v_{\theta^{t,k}} D (v_{\theta^{t,k}}-v_{\theta^{\star}})-2\beta (\theta^{t,k}-\theta^\star)^\top\nabla v_{\theta^{t,k}} D (v_{w^\star}-v_{w^{t+1}}) \nonumber \\
& +\beta^2\norm{\nabla v_{\theta^{t,k}} D (v_{\theta^{t,k}}-v_{w^{t+1}})}^2,
\end{align}
where the last equality follows from the fact that $v_{\theta^{\star}} = v_{w^{\star}}$ since $(\theta^{\star} , w^{\star}) \in \mathcal{F}_{value}$. Now, using the $F_{w}$-strong convexity of the function $w \rightarrow H(\theta^{\star} , w)$, yields
\begin{align} \label{eqn:s_proof1-temp}
 F_w\left\|\theta^{t,k}-\theta^\star\right\|^2 & \leq \left(\nabla_w H\left(\theta^\star, \theta^{t,k}\right)-\nabla_w H\left(\theta^\star, \theta^\star\right)\right)^{\top}\left(\theta^{t,k}-\theta^\star\right) \nonumber\\
 & = \nabla_w H\left(\theta^\star, \theta^{t,k}\right)^{\top}\left(\theta^{t,k}-\theta^\star\right) \nonumber \\
 & = 2(\theta^{t,k}-\theta^\star)^\top\nabla v_{\theta^{t,k}} D (v_{\theta^{t,k}}-v_{\theta^\star}),
\end{align}
where the first equality follows from the fact that $v_{w^{\star}} = \mathcal{T}v_{\theta^{\star}}$ (recall that $(\theta^{\star} , w^{\star}) \in \mathcal{F}_{value}$) since $\nabla_w H\left(\theta^\star, \theta^\star\right)=2\nabla v_{\theta^{\star}} D (v_{\theta^{\star}}-\mathcal{T}v_{\theta^\star})=2\nabla v_{\theta^{\star}} D (v_{w^{\star}}-\mathcal{T}v_{\theta^\star})={\bf 0}$. Moreover, the second equality follows from similar reasoning since $v_{\theta^{\star}} = v_{w^{\star}} = \mathcal{T}v_{\theta^{\star}}$ and thus $\nabla_w H\left(\theta^\star, \theta^{t,k}\right)=2\nabla v_{\theta^{t,k}}\cdot D(v_{\theta^{t,k}}-\mathcal{T}v_{\theta^\star}) = 2\nabla v_{\theta^{t,k}}\cdot D(v_{\theta^{t,k}}-v_{\theta^\star})$. Now, using the facts that $\norm{v_{w^{t+1}} - v_{w^\star}} \leq \kappa_{1}\norm{w^{t+1} - w^{\star}}$ and $\norm{\nabla v_{\theta^{t,k}}} \leq \kappa_{1}$, we obtain
\begin{equation}\label{eqn:s_proof2-temp}
2(\theta^{t,k}-\theta^\star)^\top\nabla v_{\theta^{t,k}}\cdot D(v_{w^\star}-v_{w^{t+1}}) \leq 2\norm{\theta^{t,k}-\theta^\star}\norm{D}\kappa_1^2 \norm{w^{t+1} - w^\star}\leq 2\kappa_{1}^2 \sigma_K\norm{\theta^{t,k}-\theta^\star}\cdot \norm{\theta^{t}-\theta^\star},
\end{equation}
where the last inequality follows from Lemma \ref{lem:interm3_strong} and the fact that $\norm{D} \leq 1$ (as $D$ is the diagonal matrix of the distributions). Furthermore, using similar arguments and the fact that $v_{w^{\star}} = v_{\theta^{\star}}$, yields
\begin{align} \label{eqn:s_proof3-temp}
\norm{\nabla v_{\theta^{t,k}}D(v_{\theta^{t,k}}-v_{w^{t+1}})} & \leq \norm{\nabla v_{\theta^{t,k}}D(v_{\theta^{t,k}}-v_{\theta^\star})}+\norm{\nabla v_{\theta^{t,k}}D(v_{w^\star}-v_{w^{t+1}})} \nonumber\\
& \leq \kappa_1^2(\norm{\theta^{t,k}-\theta^{\star}}+\norm{w^{t+1} - w^\star}) \nonumber \\
& \leq \kappa_1^2(\norm{\theta^{t,k}-\theta^{\star}}+\sigma_K\norm{\theta^{t}-\theta^{\star}}).
\end{align}
Next, we use induction to show $\norm{\theta^{t,k}-\theta^\star}^2\leq \bar{\kappa}\norm{\theta^{t,0}-\theta^\star}^2$ $\forall \;k\in[K_R]$.

For $k=1$, plug \eqref{eqn:s_proof1}, \eqref{eqn:s_proof2}, \eqref{eqn:s_proof3} (with $k=0$) back to \eqref{eqn:strong_main} to obtain 
\begin{align*}
\norm{\theta^{t,1}-\theta^\star}^2=&\norm{\theta^{t,0}-\theta^\star}^2-2\beta (\theta^{t,0}-\theta^\star)^\top\nabla v_{\theta^{t,0}} D (v_{\theta^{t,0}}-v_{\theta^{\star}})-2\beta (\theta^{t,0}-\theta^\star)^\top\nabla v_{\theta^{t,0}}D(v_{w^\star}-v_{w^{t+1}})\\
+&\beta^2\norm{\nabla v_{\theta^{t,0}}D(v_{\theta^{t,0}}-v_{w^{t+1}})}^2\\
\leq & \norm{\theta^{t,0}-\theta^\star}^2-\beta F_w \left\|\theta^{t,0}-\theta^\star\right\|^2+2\beta \kappa_1^2 \sigma_K \norm{\theta^{t,0}-\theta^\star}^2+\beta^2(1+\sigma_K)^2\kappa_1^4 \norm{\theta^{t,0}-\theta^{\star}}^2\\
=&\norm{\theta^{t,0}-\theta^\star}^2-\beta\left(F_w-2\kappa_1^2\sigma_K-\beta(1+\sigma_K)^2\kappa_1^4\right)\norm{\theta^{t,0}-\theta^\star}^2\\
\leq & (1-\frac{\beta(F_w-2\kappa_1^2\sigma_K)}{2})\norm{\theta^{t,0}-\theta^\star}^2=\max\{\frac{1}{2},1-\frac{\beta(F_w-2\kappa_1^2\sigma_K)}{2}\}\norm{\theta^{t,0}-\theta^\star}^2:=\bar{\kappa}\norm{\theta^{t,0}-\theta^\star}^2.
\end{align*}
where the last inequality uses $\beta\leq \frac{F_w-2\kappa_1^2\sigma_K}{2(1+\sigma_K)^2\kappa_1^4}$ and the last equality uses $\beta\leq\frac{1}{F_w-2\kappa_1^2\sigma_K}$.

Assume $\norm{\theta^{t,k}-\theta^\star}^2\leq \bar{\kappa}\norm{\theta^{t,0}-\theta^\star}^2$, then again
plug \eqref{eqn:s_proof1}, \eqref{eqn:s_proof2}, \eqref{eqn:s_proof3} back to \eqref{eqn:strong_main} to obtain 
\begin{align*}
&\norm{\theta^{t,{k+1}}-\theta^\star}^2=\norm{\theta^{t,k}-\theta^\star}^2-2\beta (\theta^{t,k}-\theta^\star)^\top\nabla v_{\theta^{t,k}}D(v_{\theta^{t,k}}-v_{\theta^{\star}})-2\beta (\theta^{t,k}-\theta^\star)^\top\nabla v_{\theta^{t,k}}D(v_{w^\star}-v_{w^{t+1}})\\
+&\beta^2\norm{\nabla v_{\theta^{t,k}}D(v_{\theta^{t,k}}-v_{w^{t+1}})}^2\\
\leq & \norm{\theta^{t,k}-\theta^\star}^2-\beta F_w \left\|\theta^{t,k}-\theta^\star\right\|^2+2\beta \kappa_1^2 \sigma_K \norm{\theta^{t,k}-\theta^\star}\norm{\theta^{t,0}-\theta^\star}+\beta^2\kappa_1^4 (\norm{\theta^{t,k}-\theta^{\star}}+\sigma_K\norm{\theta^{t,0}-\theta^{\star}})^2\\
\leq & \norm{\theta^{t,k}-\theta^\star}^2-\beta F_w \left\|\theta^{t,k}-\theta^\star\right\|^2+2\beta \kappa_1^2 \sigma_K \norm{\theta^{t,0}-\theta^\star}^2+\beta^2\kappa_1^4 (1+\sigma_K)^2\norm{\theta^{t,0}-\theta^{\star}}^2\\
\leq & \norm{\theta^{t,0}-\theta^\star}^2-\beta F_w \left\|\theta^{t,0}-\theta^\star\right\|^2+2\beta \kappa_1^2 \sigma_K \norm{\theta^{t,0}-\theta^\star}^2+\beta^2\kappa_1^4 (1+\sigma_K)^2\norm{\theta^{t,0}-\theta^{\star}}^2\\
=&\norm{\theta^{t,0}-\theta^\star}^2-\beta\left(F_w-2\kappa_1^2\sigma_K-\beta(1+\sigma_K)^2\kappa_1^4\right)\norm{\theta^{t,0}-\theta^\star}^2\\
\leq & (1-\frac{\beta(F_w-2\kappa_1^2\sigma_K)}{2})\norm{\theta^{t,0}-\theta^\star}^2=\max\{\frac{1}{2},1-\frac{\beta(F_w-2\kappa_1^2\sigma_K)}{2}\}\norm{\theta^{t,0}-\theta^\star}^2,
\end{align*}
where the second inequality uses $\norm{\theta^{t,k}-\theta^\star}^2\leq \bar{\kappa}\norm{\theta^{t,0}-\theta^\star}^2\leq \norm{\theta^{t,0}-\theta^\star}^2$, and the third inequality uses $\beta<1/F_w$, the last inequality uses $\beta\leq \frac{F_w-2\kappa_1^2\sigma_K}{2(1+\sigma_K)^2\kappa_1^4}$ and the last equality uses $\beta<\frac{1}{F_w}\leq\frac{1}{F_w-2\kappa_1^2\sigma_K}$.


Lastly, we choose $k=K_R$ and apply $\theta^{t,k}=\theta^{t+1}$ and $\theta^{t,0}=\theta^t$ to finish the proof.
\end{proof}


\begin{remark}
Combining Lemma~\ref{lem:interm3_strong} and under the same condition as Theorem~\ref{thm:interm3_strong-M}, we obtain $\norm{w^t-w^\star}$ also attains geometrically decay since 
\[
\left\|w^{t+1}-w^{\star}\right\| \leq \sigma_K\left\|\theta^t-\theta^{\star}\right\|\leq \sigma_K\cdot(\bar{\kappa})^{t-1}\norm{\theta^0-\theta^\star}.
\]
%\Ming{Obtaining a contraction for $\norm{w^t-w^\star}$ is harder since it is not straightforward to upper bound $\norm{\theta^t-\theta^\star}$ by $\norm{w^t-w^\star}$. Usually the term $\norm{\theta^{t-1}-\theta^\star}$ will occur.}
\end{remark}

% \begin{proposition}
% Suppose $H(\theta^\star,\cdot)$ is $F_w$ strongly convex, i.e. $\forall w_1,w_2$ $H(\theta,w_1)\geq H(\theta,w_2)+\nabla_w H(\theta,w_2)^\top(w_1-w_2)+\frac{F_w}{2}\norm{w_1-w_2}_2$,
% then 
% \[
% \mathcal{V}=\mathcal{R}'=\{(\theta^\star,w^\star)|v_{\theta^\star}=v_{w^\star},w^\star=\argmin_w H(\theta^\star,w)\}.
% \]
% \Ming{In general, we cannot guarantee $\mathcal{V}=\mathcal{R}$ under strong convexity since in this case we might not even have $H(\theta^\star,w^\star)=0$.}
% \end{proposition}

% \begin{proof}
% The proof comes from by picking $\theta=\theta^\star$ and $w_2=w^\star$ in the strongly convex condition, and this implies $H(\theta^\star,w)\geq H(\theta^\star,w^\star)$ for all $w$. 
% \end{proof}


\begin{proposition}
    
As $t\rightarrow\infty$,
\[
\norm{v_{\theta^t}-v_{w^t}} \leq (1+\sigma_K)\kappa_1(\sqrt{\bar{\kappa}})^{t-1}\norm{\theta^0-\theta^\star}\rightarrow 0.
\]
In addition, we also have
\[
\norm{v_{w^t}-\mathcal{T}v_{\theta^t}} \leq (\gamma+\sigma_K)\kappa_1(\sqrt{\bar{\kappa}})^{t-1}\norm{\theta^0-\theta^\star}\rightarrow 0,
\]
and 
\begin{equation*}
    \norm{\nabla_{w} H(\theta^{t},w^{t})} \leq  (F_{\theta}\sigma_{K} + L\sqrt{{\bar \kappa}})(\sqrt{\bar{\kappa}})^{t-2}\norm{\theta^{0}-\theta^{\star}}\rightarrow 0
\end{equation*}
\end{proposition}

\begin{proof}
For the first part of the proof, we have 
\begin{align*}
\norm{v_{\theta^t}-v_{w^t}}=&\norm{v_{\theta^t}-v_{\theta^\star}+v_{w^\star}-v_{w^t}}\leq \norm{v_{\theta^t}-v_{\theta^\star}}+\norm{v_{w^\star}-v_{w^t}}\\
\leq&\kappa_1(\norm{\theta^t-\theta^\star}+\norm{w^\star-w^t})\leq (1+\sigma_K)\kappa_1\norm{\theta^t-\theta^\star}\\
\leq& (1+\sigma_K)\kappa_1(\sqrt{\bar{\kappa}})^{t-1}\norm{\theta^0-\theta^\star}\rightarrow 0.
\end{align*}
where the third inequality uses Lemma 5.3. 
For the second part of the proof,
\begin{align*}
\norm{v_{w^t}-\mathcal{T}v_{\theta^t}}=&\norm{v_{w^t}-v_{w^\star}+\mathcal{T}v_{\theta^\star}-\mathcal{T}v_{\theta^t}}\leq \norm{v_{w^\star}-v_{w^t}}+\gamma\norm{v_{\theta^t}-v_{\theta^\star}}\\
\leq&\kappa_1(\gamma\norm{\theta^t-\theta^\star}+\norm{w^\star-w^t})\leq (\gamma+\sigma_K)\kappa_1\norm{\theta^t-\theta^\star}\\
\leq& (\gamma+\sigma_K)\kappa_1(\sqrt{\bar{\kappa}})^{t-1}\norm{\theta^0-\theta^\star}\rightarrow 0.
\end{align*}

For the last part of the proof follows
\begin{align*}
    \norm{\nabla_{w} H(\theta^{t},w^{t})} & = \norm{\nabla_{w} H(\theta^{t},w^{t}) - \nabla_{w} H(\theta^{t},w^{\star}) + \nabla_{w} H(\theta^{t},w^{\star}) - \nabla_{w} H(\theta^{\star},w^{\star})}\\ 
    & \leq \norm{\nabla_{w} H(\theta^{t},w^{t}) - \nabla_{w} H(\theta^{t},w^{\star})} + \norm{\nabla_{w} H(\theta^{t},w^{\star}) - \nabla_{w} H(\theta^{\star},w^{\star})}\\ 
    & \leq F_{\theta}\norm{w^{t} - w^{\star}} + L_w\norm{\theta^{t}-\theta^{\star}}. 
\end{align*}
Moreover from Lemma~\ref{lem:interm3_strong} we know that
\[
\left\|w^{t+1}-w^{\star}\right\| \leq \sigma_K\left\|\theta^t-\theta^{\star}\right\|
\]
and therefore it follows from Theorem~\ref{thm:interm3_strong-M} that
\begin{align*}
    \norm{\nabla_{w} H(\theta^{t},w^{t})} \leq & F_{\theta}\sigma_{K}\norm{\theta^{t - 1}-\theta^{\star}} + L\norm{\theta^{t}-\theta^{\star}} \leq (F_{\theta}\sigma_{K} + L\sqrt{{\bar \kappa}})\norm{\theta^{t - 1}-\theta^{\star}}\\
    \leq & (F_{\theta}\sigma_{K} + L\sqrt{{\bar \kappa}})(\sqrt{\bar{\kappa}})^{t-2}\norm{\theta^{0}-\theta^{\star}}\rightarrow 0
\end{align*}



\end{proof}

\section{Old result in Appendix D}


\begin{theorem}\label{thm:interm3_strong-M}
Let $\left\{ (\theta^{t} , w^{t}) \right\}_{t \in \mathbb{N}}$ be a sequence generated by the Lookahead-Replicate algorithm with $K_R=1$ and let $(\theta^{\star} , w^{\star}) \in \mathcal{F}_{value}$, i.e., $v_{w^{\star}} = \mathcal{T}v_{\theta^{\star}}$ and $v_{\theta^{\star}} = v_{w^{\star}}$. If $F_w>\max\{F_\theta, (8d+\frac{1}{d}+2)\kappa_1^2,8\kappa_1^2\}$
and the learning rate $\beta = \min\{d,\frac{C}{8D}-\sqrt{(\frac{C}{8D})^2-\frac{1}{8}}\}/\kappa_1^2$ for the Replicate steps, then
\[
(\norm{\theta^{t+1}-\theta^\star}^2+\norm{w^{t+1}-w^\star}^2)\leq \bar{\kappa}(\norm{\theta^{t}-\theta^\star}^2+\norm{w^{t}-w^\star}^2),
\]
with $\bar{\kappa}=\max\{1-\frac{1}{16}\eta^2,1-\frac{1}{8}(1-a)\}<1$. Here $d=\frac{2(1-a)}{\sqrt{a^2+8a(1-a)}+a}>0$, $a=(1-\kappa)^{K_L}$, $\eta := F_w^{-1} F_\theta$, $C=( F_w-\kappa_1^2G)/\kappa_1^2$, and $G=1+\eta^2(1-a)$.
\end{theorem}


\begin{proof}
First note that $\nabla_w \norm{v_{w}-\mathcal{T}v_{\theta}}_\rho^2=2\nabla v_w D (v_w-\mathcal{T}v_\theta)$, where $\nabla v_w\in\RR^{d\times S},D=\text{diag}(\rho)\in\RR^{S\times S},v_w-\mathcal{T}v_\theta\in\RR^{S\times 1}$. Similarly, $\nabla_\theta \norm{v_{w}-v_{\theta}}_\rho^2=2\nabla v_\theta D (v_w-v_\theta)$.

According to Algorithm Replicate($w,\theta,K$), we have that $\theta^{t+1} = \theta^{t} - 2\beta\cdot \nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{w^{t+1}})$. Using this relation yields the following
\begin{align} \label{eqn:strong_main}
\norm{\theta^{t+1}-\theta^\star}^2 & = \norm{\theta^{t}-\theta^\star - 2\beta\cdot \nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{w^{t+1}})}^2 \nonumber\\
& =\norm{\theta^{t}-\theta^\star}^2-4\beta (\theta^{t}-\theta^\star)^\top \nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{w^{t+1}})+4\beta^2\norm{\nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{w^{t+1}})}^2 \nonumber \\
& =\norm{\theta^{t}-\theta^\star}^2-4\beta (\theta^{t}-\theta^\star)^\top\nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{\theta^{\star}})-4\beta (\theta^{t}-\theta^\star)^\top\nabla v_{\theta^{t}} D (v_{w^\star}-v_{w^{t+1}}) \nonumber \\
& +4\beta^2\norm{\nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{w^{t+1}})}^2,
\end{align}
where the last equality follows from the fact that $v_{\theta^{\star}} = v_{w^{\star}}$ since $(\theta^{\star} , w^{\star}) \in \mathcal{F}_{value}$. Next, we first bound the three terms on the right hand side separately, and plug them back later.

Now, using the $F_{w}$-strong convexity of the function $w \rightarrow H(\theta^{\star} , w)$, yields
\begin{align} \label{eqn:s_proof1}
 F_w\left\|\theta^{t}-\theta^\star\right\|^2 & \leq \left(\nabla_w H\left(\theta^\star, \theta^{t}\right)-\nabla_w H\left(\theta^\star, \theta^\star\right)\right)^{\top}\left(\theta^{t}-\theta^\star\right) \nonumber\\
 & = \nabla_w H\left(\theta^\star, \theta^{t}\right)^{\top}\left(\theta^{t}-\theta^\star\right) \nonumber \\
 & = 2(\theta^{t}-\theta^\star)^\top\nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{\theta^\star}),
\end{align}
where the first equality follows from the fact that $\nabla_w H\left(\theta^\star, \theta^\star\right)=2\nabla v_{\theta^{\star}} D (v_{\theta^{\star}}-\mathcal{T}v_{\theta^\star})=2\nabla v_{\theta^{\star}} D (v_{w^{\star}}-\mathcal{T}v_{\theta^\star})={\bf 0}$, since $(\theta^{\star} , w^{\star}) \in \mathcal{F}_{value}$ and $v_{w^{\star}} = \mathcal{T}v_{\theta^{\star}}$. The second equal sign comes from
$
\nabla_w H\left(\theta^\star, \theta^{t}\right)=2\nabla v_{\theta^{t}}\cdot D(v_{\theta^{t}}-\mathcal{T}v_{\theta^\star}).
$
Next, recall $\kappa_1$ satisfies $\theta_1,\theta_2\in\Theta$, $\max_s|v_{\theta_1}(s)-v_{\theta_2}(s)|\leq \kappa_1 \norm{\theta_1-\theta_2}$ and the diagonal of $D$ is a probability distribution, we have
NO\begin{equation}\label{eqn:s_proof2}
 4\beta(\theta^{t}-\theta^\star)^\top\nabla v_{\theta^{t}}\cdot D(v_{w^\star}-v_{w^{t+1}}) \leq 4\beta\norm{\theta^{t}-\theta^\star}\cdot \kappa_1^2 \norm{w^{t+1}-w^\star} \leq  2\beta\kappa_1^2(\norm{\theta^{t}-\theta^\star}^2+  \norm{w^{t+1}-w^\star}^2),
\end{equation}
where the second inequality uses the simple fact that $2ab\leq a^2+b^2$ for any $a,b \in \mathbb{R}$. Furthermore, 
\begin{align} \label{eqn:s_proof3}
4\beta^2\norm{\nabla v_{\theta^{t}}D(v_{\theta^{t}}-v_{w^{t+1}})}^2 & \leq 8\beta^2(\norm{\nabla v_{\theta^{t}}D(v_{\theta^{t}}-v_{\theta^\star})}^2+\norm{\nabla v_{\theta^{t}}D(v_{w^\star}-v_{w^{t+1}})}^2) \nonumber \\
& \leq 8\beta^2\kappa_1^4(\norm{\theta^{t}-\theta^{\star}}^2+\norm{w^{t+1}-w^\star}^2),
\end{align}
where the first inequality uses $(a+b)^2\leq 2a^2+2b^2$. Therefore, by integrating the bounds found in \eqref{eqn:s_proof1}, \eqref{eqn:s_proof2}, and \eqref{eqn:s_proof3} back into \eqref{eqn:strong_main}, we obtain 
\begin{align}
\norm{\theta^{t+1}-\theta^\star}^2 & = \norm{\theta^{t}-\theta^\star}^2-4\beta (\theta^{t}-\theta^\star)^\top\nabla v_{\theta^{t}} D (v_{\theta^{t}}-v_{\theta^{\star}})-4\beta (\theta^{t}-\theta^\star)^\top\nabla v_{\theta^{t}}D(v_{w^\star}-v_{w^{t+1}}) \nonumber \\
& + 4\beta^2\norm{\nabla v_{\theta^{t}}D(v_{\theta^{t}}-v_{w^{t+1}})}^2 \nonumber \\
& \leq \norm{\theta^{t}-\theta^\star}^2-2\beta F_w \left\|\theta^{t}-\theta^\star\right\|^2+ (2\beta\kappa_1^2 + x8\beta^2\kappa_1^4)\left(\norm{\theta^{t}-\theta^\star}^2+ \norm{w^\star-w^{t+1}}^2\right) \nonumber \\
& =\left(1-2\beta F_w+2\beta\kappa_1^2+8\beta^2\kappa_1^4\right)\left\|\theta^t-\theta^{\star}\right\|^2+\left(8\kappa_1^4\beta^2+2\kappa_1^2\beta\right)\left\|w^{t+1}-w^{\star}\right\|^2 \nonumber \\
& \leq \left(1-2\beta F_w+2\beta\kappa_1^2+8\beta^2\kappa_1^4\right)\left\|\theta^t-\theta^{\star}\right\|^2  +\left(8\kappa_1^4\beta^2+2\kappa_1^2\beta\right)\left(a\left\|w^{t}-w^{\star}\right\|^2+\eta^2 \left(1-a\right)\left\|\theta^t-\theta^{\star}\right\|^2\right) \nonumber \\
& =\left(1-2\beta F_w+2\beta\kappa_1^2(1 +4\beta\kappa_1^2)[1+\eta^2 (1-a)]\right)\left\|\theta^t-\theta^{\star}\right\|^2  +2a\kappa_1^2\beta\left(1 + 4\beta\kappa_1^2\right)\left\|w^{t}-w^{\star}\right\|^2,  \label{eqn:key1}
\end{align}
where the second inequality follows from Lemma \ref{lem:interm3_strong}.




Now we combine 
\eqref{eqn:key1} + \eqref{eqn:key2} to obtain 
\[
\norm{\theta^{t+1}-\theta^\star}+\norm{w^{t+1}-w^\star}\leq E \norm{\theta^{t}-\theta^\star}+F \norm{w^{t}-w^\star}
\]

where we need 
\[
0\leq E:=1-2\beta F_w+2\beta\kappa_1^2[1+\eta^2 (1-a)]+8\beta^2\kappa_1^4[1+\eta^2 (1-a)]+\eta^2(1-a)\leq 1-\frac{1}{16}\eta^2
\]
and
\[
0\leq F:=8a\kappa_1^4\beta^2+2a\kappa_1^2\beta + a\leq 1-\frac{1}{8}(1-a)
\]

\textbf{Step 1.} First note $0\leq F$ holds naturally. We next solve $F\leq 1-\frac{1}{8}(1-a)$. Define $\kappa_1^2\beta=x$, then we have $8ax^2+2ax+\frac{7}{8}(a-1)\leq 0$. The positive root is $\frac{7(1-a)}{8(\sqrt{a^2+7a(1-a)}+a)}$ (the other root is negative), so it needs to satisfy
\begin{equation}\label{eqn:234}
\beta \kappa_1^2\leq \frac{7(1-a)}{8(\sqrt{a^2+7a(1-a)}+a)}:=d.
\end{equation}


\textbf{Step 2.} We further solve $0\leq E\leq 1-\frac{1}{16}\eta^2$. For convenience, let us denote 
\[
G:=1+\eta^2(1-a),
\]
then we have
\[
E=-2\beta F_w+2\beta\kappa_1^2G+8\beta^2\kappa_1^4G+G
\]
As a result, denote $C=( F_w-\kappa_1^2G)/\kappa_1^2$ and $x=\beta\kappa_1^2$ we have
\begin{equation}\label{eqn:01}
\begin{aligned}
&0\leq E\leq 1-\frac{1}{16}\eta^2\\
\Leftrightarrow &0\leq -2\beta F_w+2\beta\kappa_1^2G+8\beta^2\kappa_1^4G+G\leq 1-\frac{1}{16}\eta^2\\
\Leftrightarrow& 0\leq -2\beta( F_w-\kappa_1^2G)+8\beta^2\kappa_1^4G+G\leq 1-\frac{1}{16}\eta^2\\
\Leftrightarrow& 0\leq -2Cx+8Gx^2+G\leq 1-\frac{1}{16}\eta^2\\
\Leftrightarrow& 0\leq x^2-2\frac{C}{8G}x+\frac{1}{8}\leq \frac{1-\frac{1}{16}\eta^2}{8G}\\
\Leftrightarrow& 0\leq x^2-2\frac{C}{8G}x+(\frac{C}{8G})^2-(\frac{C}{8G})^2+\frac{1}{8}\leq \frac{1-\frac{1}{16}\eta^2}{8G}\\
\Leftrightarrow& (\frac{C}{8G})^2-\frac{1}{8}\leq (x-\frac{C}{8G})^2\leq \frac{1-\frac{1}{16}\eta^2}{8G}+(\frac{C}{8G})^2-\frac{1}{8}\\
\Leftrightarrow& \sqrt{(\frac{C}{8G})^2-\frac{1}{8}}\leq |x-\frac{C}{8G}|\leq \sqrt{\frac{1-\frac{1}{16}\eta^2}{8G}+(\frac{C}{8G})^2-\frac{1}{8}}\\
\Leftarrow& \frac{C}{8G}-\sqrt{\frac{1-\frac{1}{16}\eta^2}{8G}+(\frac{C}{8G})^2-\frac{1}{8}}\leq x\leq \frac{C}{8G}-\sqrt{(\frac{C}{8G})^2-\frac{1}{8}}
\end{aligned}
\end{equation}
Here we use the condition 
\[
F_w\geq 8\kappa_1^2> (1+\sqrt{8})\kappa_1^2G\Leftrightarrow (\frac{C}{8G})^2-\frac{1}{8}\geq 0
\]
so $\sqrt{(\frac{C}{8G})^2-\frac{1}{8}}$ is valid.



Therefore, via \eqref{eqn:234} and \eqref{eqn:01} we only require 
\begin{equation}\label{eqn:666}
 \frac{C}{8G}-\sqrt{\frac{1-\frac{1}{16}\eta^2}{8G}+(\frac{C}{8G})^2-\frac{1}{8}}\leq d
\end{equation}
If $d\geq \frac{C}{8G}$, the above is automatically satisfied;
If $d< \frac{C}{8G}$, then above is equivalent to 
\begin{align*}
    &\frac{C}{8G}-d\leq \sqrt{\frac{1-\frac{1}{16}\eta^2}{8G}+(\frac{C}{8G})^2-\frac{1}{8}}\\
    \Leftrightarrow&(\frac{C}{8G}-d)^2\leq \frac{1-\frac{1}{16}\eta^2}{8G}+(\frac{C}{8G})^2-\frac{1}{8}\\
    \Leftrightarrow&(\frac{C}{8G})^2-\frac{C}{4G}d+d^2\leq \frac{1-\frac{1}{16}\eta^2}{8G}+(\frac{C}{8G})^2-\frac{1}{8}\\
    \Leftrightarrow& d^2+\frac{1}{8}-\frac{1-\frac{1}{16}\eta^2}{8G}\leq  \frac{C}{4G}d\\
    \Leftarrow & \frac{4G}{d}(d^2+\frac{1}{8})\leq C\Leftarrow  \frac{8}{d}(d^2+\frac{1}{8})\leq C\\
    \Leftrightarrow & 8d+\frac{1}{d}\leq C\\
    \Leftrightarrow & (8d+\frac{1}{d}+G)\kappa_1^2\leq F_w\\
        \Leftarrow & (8d+\frac{1}{d}+2)\kappa_1^2\leq F_w
\end{align*}
Therefore, as long as $(8d+\frac{1}{d}+2)\kappa_1^2\leq F_w$ is satisfied, the condition \eqref{eqn:666} is true.

Therefore, we can choose 
\[
x = \min\{d,\frac{C}{8G}-\sqrt{(\frac{C}{8G})^2-\frac{1}{8}}\}
\]
which is
\[
\beta = \min\{d,\frac{C}{8G}-\sqrt{(\frac{C}{8G})^2-\frac{1}{8}}\}/\kappa_1^2
\]
to obtain that 
\[
(\norm{\theta^{t+1}-\theta^\star}^2+\norm{w^{t+1}-w^\star}^2)\leq \bar{\kappa}(\norm{\theta^{t}-\theta^\star}^2+\norm{w^{t}-w^\star}^2)
\]
with $\bar{\kappa}=\max\{1-\frac{1}{16}\eta^2,1-\frac{1}{8}(1-a)\}<1$.
\end{proof}
